A Simple NLP-based Approach to Support Onboarding and Retention in Open Source Communities

Successful open source communities are constantly looking for new members and helping them become active developers. A common approach for developer onboarding in open source projects is to let newcomers focus on relevant yet easy-to-solve issues to familiarize themselves with the code and the community. The goal of this research is twofold. First, we aim at automatically identifying issues that newcomers can resolve by analyzing the history of resolved issues by simply using the title and description of issues. Second, we aim at automatically identifying issues, that can be resolved by newcomers who later become active developers. We mined the issue trackers of three large open source projects and extracted natural language features from the title and description of resolved issues. In a series of experiments, we optimized and compared the accuracy of four supervised classifiers to address our research goals. Random Forest, achieved up to 91% precision (F1-score 72%) towards the first goal while for the second goal, Decision Tree achieved a precision of 92% (F1-score 91%). A qualitative evaluation gave insights on what information in the issue description is helpful for newcomers. Our approach can be used to automatically identify, label, and recommend issues for newcomers in open source software projects based only on the text of the issues.

==> listings/classification_pseudo_code.tex <==
\begin{algorithm}
    \small
    \caption{Classification Procedure}
    \label{alg:classification}
    \begin{algorithmic} 
        \REQUIRE The first $t$ issues addressed by $nc_t$ with $t \in \{1, 5, 10\}$ are marked for the classification
        \STATE {projects $\leftarrow$ [QT , Eclipse, LibreOffice]}
        \STATE {classifiers $\leftarrow$ [Random Forest , GaussianNB, DecisionTree, LIBSMV]}
        \STATE {$n\_runs \leftarrow 5$}
        \FORALL{projects} 
            \STATE{project $\leftarrow$ load file including machine learning features}
            \FORALL{classifiers}
                \STATE{grid $\leftarrow$ set hyper-parameter ranges for classifier}
                \FOR{$i = 0$ \TO $n\_runs$}
                    \STATE{data\_true\_class $\leftarrow$ extract from data source}
                    \STATE{data\_false\_class $\leftarrow$ extract from data source}
                    \STATE{data\_false\_class $\leftarrow$ under-sample}    \STATE{dataset $\leftarrow$ data\_true\_class $+$ data\_false\_class}
                    \STATE{}
                    \STATE{train, test $\leftarrow$ split dataset (15\% to the test set)}
                    \STATE{}
                    \STATE{oversampled\_data $\leftarrow$ over-sample data\_true\_class from the train data}
                    \STATE{train $\leftarrow$ append oversampled\_data}
                    \STATE{}
                    \STATE{grid\_results $\leftarrow$ 10-cross-fold validation}
                    \STATE{clf $\leftarrow$ build classifier with the best hyper-parameters using the train data}
                    \STATE{precision, recall, F1-score $\leftarrow$ clf predicting the test data}
                    \STATE{csv $\leftarrow$ store the results}
                \ENDFOR
            \ENDFOR
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

==> sections/drafting.tex <==
Paper narrative

References can be found here

- One of the barrier to OSS participation is``the difficulty for newcomers to find an appropriate item to work on'' (SSG15)
- In this study we want to find what are the characteristics of an issue that can be taken on by a newcomer
  - (Binary) categorization problem: newbie-friendly vs newbie-unfriendly issues -> Issues fixed by first (second, third, etc) committer vs. Issues fixed by experienced committer
  - NLP-based classifier predicting whether a feature is likely to be take on by a newcomer or not
  - Feature selection on the model to characterized the issue
- Contribution: Guidelines to write attractive bug reports for newbies (?)

Most relevant papers

- DSS13:
  - Characterize the behavior of committers based on several metrics (mostly code-based).
  - Finds four classes Core, Active, Occasional, and Rare developers.
    - This seems important to us. Perhaps we could use their definition of Core and Active as our target.
  - PCA + FA + Cluster analysis.
  - Interpretation of PCA factors: Programming activity, Inter-commit time, Extent of contribution.
- LH15:
  - Study of GFB by Mozilla (67% first attempt success rate).
  - First time committers satisfied with the program.
  - GFB does not improve newbie likelihood to make a contribution. Those who do not turn into long-time committers -> Better way to assess newbie-friendly issue.
- SCG15:
  - Grounded theory on problems newbies face when picking the first issue to work on.
  - Suggests two (WS11 and CMS05) tools based on project artifact that reconstruct the context of the issue and help the newbie -> Recommend existing issues rather than helping in writing newbie-friendly ones.
  - Suggests mentoring approach -> No good (see LH15)

Problems:

- characterize newcomer (e.g., time between creating account and first submission)
- missing information about the newcomer previous knowledge

Misc:

- Mozilla projects have a special keyword (good-first-bug) for tagging newbie-friendly item in their tracker
- There is an IBM paper (MSA18) which uses deep learning for triaging. Basically theirs is a general case of ours. Can we reuse it?


==> sections/metacontent.tex <==
`%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10003120.10003130.10003233.10003597</concept_id>
<concept_desc>Human-centered computing~Open source software</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003130.10003131.10003270</concept_id>
<concept_desc>Human-centered computing~Social recommendation</concept_desc>
<concept_significance>400</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003130.10003131.10003376</concept_id>
<concept_desc>Human-centered computing~Social tagging</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003130.10003131.10003235</concept_id>
<concept_desc>Human-centered computing~Collaborative content creation</concept_desc>
<concept_significance>300</concept_significance>
</concept>
<concept>
<concept_id>10003120.10003130.10003131.10003570</concept_id>
<concept_desc>Human-centered computing~Computer supported cooperative work</concept_desc>
<concept_significance>100</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Human-centered computing~Open source software}
\ccsdesc[400]{Human-centered computing~Social recommendation}
\ccsdesc[300]{Human-centered computing~Social tagging}
\ccsdesc[300]{Human-centered computing~Collaborative content creation}
\ccsdesc[100]{Human-centered computing~Computer supported cooperative work}

\keywords{open source software, onboarding, retention, issue, classification, machine learning}

==> table/data_balance.tex <==
\begin{table}[tb]
\centering
\footnotesize
\caption{Number of issues belonging to each class. For RQ1: resolved by newcomer\textbf{:}other issues. For RQ2: resolved by newcomer who retained\textbf{:}newcomer that quit.}
\label{tab:data-balance}
\begin{tabular}{l|ccc|c}
\toprule
                    & \multicolumn{3}{c|}{\textbf{RQ1}}         & \textbf{RQ2} \\ 
\textbf{Project}    & $nc_1$       & $nc_5$      & $nc_{10}$      & $nc_1$ \\ \midrule
Qt                  & 777\textbf{:}53714    & 1836\textbf{:}52654  & 2941\textbf{:}51549   & 159\textbf{:}617 \\
Eclipse             & 3020\textbf{:}153707  & 7977\textbf{:}148750 & 11989\textbf{:}144738 & 450\textbf{:}2570 \\
LibreOffice         & 457\textbf{:}10438    & 700\textbf{:}10195   & 900\textbf{:}9995     & 76\textbf{:}381 \\ \bottomrule
\end{tabular}
\end{table}
